New LZ and PW(Z) relations of RR Lyrae stars calibrated with Gaia EDR3 parallaxes

We present new luminosity-metallicity (LZ; MV-[Fe/H] and MG-[Fe/H]) relations and, for the first time, empirical, Gaia three-band (G,GBP,GRP) period-Wesenheit-metallicity (PWZ) relations of RR Lyrae stars (RRLs) derived using a hierarchical Bayesian approach and new accurate parallaxes published for these variables in the Gaia Early Data Release 3 (EDR3). In a previous study we obtained Bayesian hierarchically-derived LZ relations from a sample of about four hundred Milky Way field RRLs with G-band light curves and trigonometric parallaxes published in the Gaia Data Release 2 (DR2), using V mean magnitudes, metallicities, absorptions and pulsation periods available in the literature. We now extend that study in two directions. Firstly, we update our previous results using trigonometric parallaxes from Gaia EDR3 and incorporate the Bayesian analysis of a first empirical PWZ relation derived using those field RRLs with G, GBP and GRP time-series photometry available in Gaia DR2. Secondly, we use Bayesian inference to derive LZ relations and empirical PW Gaia three-band relations from 385 RRLs belonging to 15 Milky Way globular clusters (GC) with literature-compiled spectroscopic metallicities ranging from -0.36 to -2.39 dex and prior distances extending from 2.2 to 41.2 kpc. From the samples of RRLs analysed in this paper we infer a mean Gaia EDR3 zero-point offset of -0.028 mas with median values ranging from -0.033 (LZ and PWZ models for field stars) to -0.024 mas (LZ model in the V-band for GC RRLs).

==> LZ-G-Band-GC-PL-EDR3.tex <==
% latex table generated in R 3.4.3 by xtable 1.8-4 package
% Thu Feb 18 10:26:55 2021
\begin{table*}
\centering
\caption{ {\bf (2nd update by  HED) } Summary statistics of the population-level RRL parameters inferred by the $M_{G}-[\mathrm{Fe/H}]$ HM. Each parameter is named as in Table \ref{tab:V-FeH-GC-PL}.} 
\label{tab:G-FeH-GC-PL}
\begin{tabular}{llll}
  \hline
%  & $\gamma_{1}$ & $\gamma_{0}$ & $\tau$ & $\Delta\varpi$ & $\mu_{\rm{LMC}}$ \\ 
  
  \multicolumn{1}{c}{$\gamma_{1}$} & \multicolumn{1}{c}{$\gamma_{0}$} & 
     \multicolumn{1}{c}{$\tau$} & \multicolumn{1}{c}{${\Delta\varpi}_{0}$}  \\
     \multicolumn{1}{c}{(mag/dex)}   & \multicolumn{1}{c}{(mag)}  & \multicolumn{1}{c}{(mag)}    & \multicolumn{1}{c} {(mas)}  \\

  
  
  
  \hline
$0.28_{-0.36}^{+0.36}$ & $0.97_{-0.52}^{+0.49}$ & $0.131_{-0.095}^{+0.183}$ & $-0.028_{-0.008}^{+0.009}$ \\ 
   \hline
\end{tabular}
\end{table*}


==> LZ-V-Band-GC-PL-EDR3.tex <==
% latex table generated in R 3.4.3 by xtable 1.8-4 package
% Thu Feb 18 10:36:38 2021
\begin{table*}
\centering
\caption{ {\bf (2nd update by HED)} Summary statistics of the population-level RRL parameters inferred by the
                             $M_{V}-[\mathrm{Fe/H}]$ HM. $\gamma_{1}$, $\gamma_{0}$ and $\tau$  represent the slope, the intercept and the dispersion of the the linear relationship  between the mean globular cluster RRL absolute magnitude $\beta_{0}$ and $[\rm{Fe/H}]$ according to Eq. \eqref{eq:beta-distr-LZ}, respectively. $\Delta\varpi_{0}$ denotes the parallax zero-point offset calculated as described in the text}. 
\label{tab:V-FeH-GC-PL}
\begin{tabular}{llll}
  \hline
%  & $\gamma_{1}$ & $\gamma_{0}$ & $\tau$ & $\Delta\varpi$ & $\mu_{\rm{LMC}}$ \\ 
  
   \multicolumn{1}{c}{$\gamma_{1}$} & \multicolumn{1}{c}{$\gamma_{0}$} & 
     \multicolumn{1}{c}{$\tau$} & \multicolumn{1}{c}{${\Delta\varpi}_{0}$} \\
     \multicolumn{1}{c}{(mag/dex)}   & \multicolumn{1}{c}{(mag)}  & \multicolumn{1}{c}{(mag)}    & \multicolumn{1}{c} {(mas)}   \\

  
  
  \hline
  $0.29_{-0.29}^{+0.35}$ & $1.05_{-0.46}^{+0.43}$ & $0.108_{-0.080}^{+0.154}$ & $-0.024_{-0.008}^{+0.008}$   \\ 
   \hline
\end{tabular}
\end{table*}

